The Kemeny constant of a Markov chain

Given an ergodic finite-state Markov chain, let M_{iw} denote the mean time from i to equilibrium, meaning the expected time, starting from i, to arrive at a state selected randomly according to the equilibrium measure w of the chain. John Kemeny observed that M_{iw} does not depend on starting the point i. The common value K=M_{iw} is the Kemeny constant or seek time of the chain. K is a spectral invariant, to wit, the trace of the resolvent matrix. We review basic facts about the seek time, and connect it to the bus paradox and the Central Limit Theorem for ergodic Markov chains.

==> kc_dot_bib <==
@unpublished {Aldousfill,
	AUTHOR={Aldous, David and Fill, Jim},
	TITLE={Reversible Markov Chains and Random Walks on Graphs},
	NOTE={\url{http://www.stat.berkeley.edu/users/aldous/RWG/book.html}},
	YEAR={2002},
}

@book {Aubin,
    AUTHOR = {Aubin, Thierry},
     TITLE = {Some nonlinear problems in {R}iemannian geometry},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin},
      YEAR = {1998},
     PAGES = {xviii+395},
      ISBN = {3-540-60752-8},
}

@article {Chiu,
    AUTHOR = {Chiu, Patrick},
     TITLE = {Height of flat tori},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {125},
      YEAR = {1997},
    NUMBER = {3},
     PAGES = {723--730},
      ISSN = {0002-9939},
     CODEN = {PAMYAR},
   MRCLASS = {58G26 (11E45)},
  MRNUMBER = {MR1396970 (97g:58173)},
MRREVIEWER = {Jack Quine},
}

@article {Diaconisstroock,
    AUTHOR = {Diaconis, Persi and Stroock, Daniel},
     TITLE = {Geometric bounds for eigenvalues of {M}arkov chains},
   JOURNAL = {Ann. Appl. Probab.},
  FJOURNAL = {The Annals of Applied Probability},
    VOLUME = {1},
      YEAR = {1991},
    NUMBER = {1},
     PAGES = {36--61},
      ISSN = {1050-5164},
   MRCLASS = {60J10},
  MRNUMBER = {MR1097463 (92h:60103)},
MRREVIEWER = {Gregory F. Lawler},
}

 @article {Morpurgo,
    AUTHOR = {Morpurgo, C.},
     TITLE = {The logarithmic {H}ardy-{L}ittlewood-{S}obolev inequality and
              extremals of zeta functions on ${S}\sp n$},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {6},
      YEAR = {1996},
    NUMBER = {1},
     PAGES = {146--171},
      ISSN = {1016-443X},
 }
 
 @article {Morpurgo_Duke,
    AUTHOR = {Morpurgo, Carlo},
     TITLE = {Sharp inequalities for functional integrals and traces of
              conformally invariant operators},
   JOURNAL = {Duke Math. J.},
  FJOURNAL = {Duke Mathematical Journal},
    VOLUME = {114},
      YEAR = {2002},
    NUMBER = {3},
     PAGES = {477--553},
      ISSN = {0012-7094},
}



@article {Ops,
    AUTHOR = {Osgood, B. and Phillips, R. and Sarnak, P.},
     TITLE = {Extremals of determinants of {L}aplacians},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {80},
      YEAR = {1988},
    NUMBER = {1},
     PAGES = {148--211},
      ISSN = {0022-1236},
 }



@article {Okikiolu,
    AUTHOR = {Okikiolu, K.},
     TITLE = {Critical metrics for the determinant of the {L}aplacian in odd
              dimensions},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {153},
      YEAR = {2001},
    NUMBER = {2},
     PAGES = {471--531},
}

@article {Okikiolububble,
    AUTHOR = {Okikiolu, K.},
     TITLE = {A negative mass theorem for the 2-torus},
       eprint = {arXiv:0711.3489v1 [math.SP]},
       YEAR={2007},
}

@article {Okikiolutrace,
    AUTHOR = {Okikiolu, K.},
     TITLE = {Extremals for logarithmic {H}ardy-{L}ittlewood-{S}obolev inequalities on compact manifolds},
       eprint = {arXiv:math/0603717v1 [math.SP]},
       YEAR={2006},
}

@article {Richardson,
    AUTHOR = {Richardson, Ken},
     TITLE = {Critical points of the determinant of the {L}aplace operator},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {122},
      YEAR = {1994},
    NUMBER = {1},
     PAGES = {52--83},
      ISSN = {0022-1236},
     CODEN = {JFUAAW},
   MRCLASS = {58G26 (58E11)},
  MRNUMBER = {95j:58176},
MRREVIEWER = {Paul C. Yang},
}


@book {Taylor1,
    AUTHOR = {Taylor, Michael E.},
     TITLE = {Partial differential equations. {I}},
    SERIES = {Applied Mathematical Sciences},
    VOLUME = {115},
      NOTE = {Basic theory},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {New York},
      YEAR = {1996},
     PAGES = {xxiv+563},
      ISBN = {0-387-94653-5},
   MRCLASS = {35-01 (46N20 47N20 58Gxx)},
  MRNUMBER = {98b:35002b},
MRREVIEWER = {Luigi Rodino},
}

@book{feller1,
author={Feller, William},
title={An Introduction to Probability Theory and its Applications {I}, 3rd ed.},
publisher={Wiley},
year={1968}
}


 @article {steiner_duke,
    AUTHOR = {Steiner, Jean},
     TITLE = {A geometrical mass and its extremal properties for metrics on {$S\sp 2$}},
   JOURNAL = {Duke Math. J.},
  FJOURNAL = {Duke Mathematical Journal},
    VOLUME = {129},
      YEAR = {2005},
    NUMBER = {1},
     PAGES = {63--86},
}



@article{hideandseek,
AUTHOR={Doyle, Peter and Steiner, Jean},
TITLE={Spectral invariants and playing hide-and-seek on surfaces},
eprint={arXiv:0904.xxxxv1 [math.SP]},
YEAR = {2005},
}

@article{skinnytori,
AUTHOR={Doyle, Peter and Steiner, Jean},
TITLE={Blowing bubbles on the torus},
eprint={arXiv:0904.xxxxv1 [math.SP]},
YEAR = {2005},
}


@article {Leveneloizou,
    AUTHOR = {Levene, Mark and Loizou, George},
     TITLE = {Kemeny's constant and the random surfer},
   JOURNAL = {Amer. Math. Monthly},
  FJOURNAL = {The American Mathematical Monthly},
    VOLUME = {109},
      YEAR = {2002},
    NUMBER = {8},
     PAGES = {741--745},
      ISSN = {0002-9890},
     CODEN = {AMMYAE},
   MRCLASS = {60J10 (60E15)},
  MRNUMBER = {MR1927624 (2003e:60162)},
MRREVIEWER = {Vivek S. Borkar},
}

@book {Kemenysnell,
    AUTHOR = {Kemeny, John G. and Snell, J. Laurie},
     TITLE = {Finite {M}arkov chains},
    SERIES = {The University Series in Undergraduate Mathematics},
 PUBLISHER = {D. Van Nostrand Co., Inc., Princeton, N.J.-Toronto-London-New
              York},
      YEAR = {1960},
     PAGES = {viii+210},
   MRCLASS = {60.00},
  MRNUMBER = {MR0115196 (22 \#5998)},
MRREVIEWER = {K. L. Chung},
}


@book {RWEN,
    AUTHOR = {Doyle, Peter and Snell, J. Laurie},
     TITLE = {Random walks and electric networks},
    SERIES = {Carus Mathematical Monographs},
    VOLUME = {22},
 PUBLISHER = {Mathematical Association of America},
   ADDRESS = {Washington, DC},
      YEAR = {1984},
     PAGES = {xiv+159},
      ISBN = {0-88385-024-9},
   MRCLASS = {94C05 (60J15 94C15)},
  MRNUMBER = {MR920811 (89a:94023)},
MRREVIEWER = {H. Kesten},
}

@article {Meyer,
    AUTHOR = {Meyer, Jr., Carl D.},
     TITLE = {The role of the group generalized inverse in the theory of
              finite {M}arkov chains},
   JOURNAL = {SIAM Rev.},
  FJOURNAL = {SIAM Review},
    VOLUME = {17},
      YEAR = {1975},
     PAGES = {443--464},
      ISSN = {1095-7200},
   MRCLASS = {60J10},
  MRNUMBER = {MR0383538 (52 \#4419)},
MRREVIEWER = {E. Seneta},
}

@book {Hsu,
    AUTHOR = {Hsu, Elton P.},
     TITLE = {Stochastic analysis on manifolds},
    SERIES = {Graduate Studies in Mathematics},
    VOLUME = {38},
 PUBLISHER = {American Mathematical Society},
   ADDRESS = {Providence, RI},
      YEAR = {2002},
     PAGES = {xiv+281},
      ISBN = {0-8218-0802-8},
   MRCLASS = {58J65 (60-02 60G48 60H05 60H10 60J60 60J65)},
  MRNUMBER = {MR1882015 (2003c:58026)},
MRREVIEWER = {Yu. E. Gliklikh},
}

@unpublished{Doyle_Kemeny,
AUTHOR={Doyle, Peter},
TITLE={Kemeny's Constant},
NOTE = {\url{ http://math.dartmouth.edu/~doyle/docs/kc/kc.pdf}}, 
YEAR = {2003},
}


@inproceedings{Lovaszwinkler,
 author = {Lovasz, Laslo and Peter Winkler},
 title = {Efficient stopping rules for Markov chains},
 booktitle = {STOC '95: Proceedings of the twenty-seventh annual ACM
symposium on Theory of computing},
 year = {1995},
 isbn = {0-89791-718-9},
 pages = {76--82},
 location = {Las Vegas, Nevada, United States},
 doi = {http://doi.acm.org/10.1145/225058.225086},
 publisher = {ACM Press},
 address = {New York, NY, USA},
 }	

@book {Grinsteadsnell,
    AUTHOR = {Grinstead, Charles M. and Snell, J. Laurie},
     TITLE = {Introduction to Probability: Second Revised Edition},
 PUBLISHER = {American Mathematical Society},
      YEAR = {1997},
     PAGES = {xi+510},
      ISBN = {0-8218-0749-8},
}

@book {kemenysnellfinite,
    AUTHOR = {Kemeny, John G. and Snell, J. Laurie},
     TITLE = {Finite {M}arkov chains},
 PUBLISHER = {Van Nostrand},
      YEAR = {1960},
}


@article {Carlenloss,
    AUTHOR = {Carlen, E. and Loss, M.},
     TITLE = {Competing symmetries, the logarithmic {H}{L}{S} inequality and
              {O}nofri's inequality on ${S}\sp n$},
   JOURNAL = {Geom. Funct. Anal.},
  FJOURNAL = {Geometric and Functional Analysis},
    VOLUME = {2},
      YEAR = {1992},
    NUMBER = {1},
     PAGES = {90--104},
      ISSN = {1016-443X},
 }

@article {Beckner,
    AUTHOR = {Beckner, William},
     TITLE = {Sharp {S}obolev inequalities on the sphere and the
              {M}oser-{T}rudinger inequality},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {138},
      YEAR = {1993},
    NUMBER = {1},
     PAGES = {213--242},
      ISSN = {0003-486X},
 }

@article {Raysinger,
    AUTHOR = {Ray, D. B. and Singer, I. M.},
     TITLE = {{$R$}-torsion and the {L}aplacian on {R}iemannian manifolds},
   JOURNAL = {Advances in Math.},
    VOLUME = {7},
      YEAR = {1971},
     PAGES = {145--210},
   MRCLASS = {58F20 (53C20)},
  MRNUMBER = {45 \#4447},
MRREVIEWER = {J. W. Robbin},
}

@article {Polyakov1,
    AUTHOR = {Polyakov, A. M.},
     TITLE = {Quantum geometry of fermionic strings},
   JOURNAL = {Phys. Lett. B},
  FJOURNAL = {Physics Letters. B},
    VOLUME = {103},
      YEAR = {1981},
    NUMBER = {3},
     PAGES = {211--213},
      ISSN = {0031-9163},
     CODEN = {PYLBA},
   MRCLASS = {81E99 (58D30 81G20 82A68)},
  MRNUMBER = {84h:81093b},
}
@article {Polyakov2,
    AUTHOR = {Polyakov, A. M.},
     TITLE = {Quantum geometry of bosonic strings},
   JOURNAL = {Phys. Lett. B},
  FJOURNAL = {Physics Letters. B},
    VOLUME = {103},
      YEAR = {1981},
    NUMBER = {3},
     PAGES = {207--210},
      ISSN = {0031-9163},
     CODEN = {PYLBA},
   MRCLASS = {81E99 (58D30 81G05 82A68)},
  MRNUMBER = {84h:81093a},
}


